Symbolic Knowledge Extraction and Injection with Sub-symbolic Predictors: A Systematic Literature Review

In this paper we focus on the opacity issue of sub-symbolic machine learning predictors by promoting two complementary activities, namely, symbolic knowledge extraction (SKE) and injection (SKI) from and into sub-symbolic predictors. We consider as symbolic any language being intelligible and interpretable for both humans and computers. Accordingly, we propose general meta-models for both SKE and SKI, along with two taxonomies for the classification of SKE and SKI methods. By adopting an explainable artificial intelligence (XAI) perspective, we highlight how such methods can be exploited to mitigate the aforementioned opacity issue. Our taxonomies are attained by surveying and classifying existing methods from the literature, following a systematic approach, and by generalising the results of previous surveys targeting specific sub-topics of either SKE or SKI alone. More precisely, we analyse 132 methods for SKE and 117 methods for SKI, and we categorise them according to their purpose, operation, expected input/output data and predictor types. For each method, we also indicate the presence/lack of runnable software implementations. Our work may be of interest for data scientists aiming at selecting the most adequate SKE/SKI method for their needs, and also work as suggestions for researchers interested in filling the gaps of the current state of the art, as well as for developers willing to implement SKE/SKI-based technologies.

==> figures/timeline-ske.tex <==
% !TeX root = ../acmcs-skeskislr.tex
% CURRENTLY NOT USED AS THE RENDERING IS AWFUL

% \usepackage{chronology}
% \usepackage{lscape}

\newcommand{\newSkeEvent}[2]{\event{#1}{\cite{#2}}}

\begin{landscape}
\begin{chronology}[10]{1980}{2022}{\textwidth}
    \newSkeEvent{1984}{breiman1984classification}
    \newSkeEvent{1986}{Quinlan86ID3}
    \newSkeEvent{1988}{SaitoN88}
    \newSkeEvent{1989}{ClarkN89}
    \newSkeEvent{1990}{Masuoka1990}
    \newSkeEvent{1990}{Hayashi90}
    \newSkeEvent{1991}{TowellS91}
    \newSkeEvent{1991}{Berenji91}
    \newSkeEvent{1991}{BrunkP91}
    \newSkeEvent{1991}{murphy1991id2}
    \newSkeEvent{1992}{HorikawaFU92}
    \newSkeEvent{1992}{TrespHA92}
    \newSkeEvent{1993}{towell1993extracting}
    \newSkeEvent{1993}{Thrun1993ExtractingPC}
    \newSkeEvent{1993}{Cohen93}
    \newSkeEvent{1993}{quinlan1993c4}
    \newSkeEvent{1994}{Fu94}
    \newSkeEvent{1994}{halgamuge1994neural}
    \newSkeEvent{1994}{MITRA1994285}
    \newSkeEvent{1994}{craven1994using}
    \newSkeEvent{1994}{FurnkranzW94}
    \newSkeEvent{1994}{sestito94automated}
    \newSkeEvent{1995}{Andrews95rulex}
    \newSkeEvent{1995}{Matthews95fuzzy}
    \newSkeEvent{1995}{Cohen95}
    \newSkeEvent{1995}{PopTHSD95}
    \newSkeEvent{1996}{SetionoL96}
    \newSkeEvent{1996}{tickle1996dedec}
    \newSkeEvent{1996}{YuanZ96}
    \newSkeEvent{1996}{craven1996extracting}
    \newSkeEvent{1996}{HongL96}
    \newSkeEvent{1997}{Setiono97NeuroLinear}
    \newSkeEvent{1997}{Setiono97a}
    \newSkeEvent{1997}{NauckK97}
    \newSkeEvent{1997}{SaitoN97}
    \newSkeEvent{1997}{BenitezCR97}
    \newSkeEvent{1997}{IshibuchiNM97}
    \newSkeEvent{1999}{TahaG99}
    \newSkeEvent{1999}{TahaG99}
    \newSkeEvent{1999}{Krishnan99combo}
    \newSkeEvent{1999}{NauckK99}
    \newSkeEvent{1999}{TahaG99}
    \newSkeEvent{1999}{KrishnanSB99}
    \newSkeEvent{1999}{schmitz1999ann}
    \newSkeEvent{1999}{HongC99}
    \newSkeEvent{2000}{Setiono00}
    \newSkeEvent{2000}{Tsukimoto00}
    \newSkeEvent{2000}{Kim2000}
    \newSkeEvent{2000}{SetionoL00}
    \newSkeEvent{2000}{ZhouCC00}
    \newSkeEvent{2000}{HongC00a}
    \newSkeEvent{2001}{sato2001rule}
    \newSkeEvent{2001}{parpinelli2001ant}
    \newSkeEvent{2001}{CastilloGP01}
    \newSkeEvent{2002}{saito2002extracting}
    \newSkeEvent{2002}{setiono2002extraction}
    \newSkeEvent{2002}{liu2002density}
    \newSkeEvent{2002}{Boz02}
    \newSkeEvent{2003}{Markowska-KaczmarT03}
    \newSkeEvent{2003}{ZhouJC03}
    \newSkeEvent{2004}{SetionoT04}
    \newSkeEvent{2004}{Fu2004}
    \newSkeEvent{2004}{Markowska-KaczmarC04}
    \newSkeEvent{2004}{RabunalDPPR04}
    \newSkeEvent{2004}{Chen2004LEARNINGAA}
    \newSkeEvent{2004}{LiuAM04}
    \newSkeEvent{2004}{Browne2004}
    \newSkeEvent{2005}{ZhangSJC05}
    \newSkeEvent{2005}{barakat2005eclectic}
    \newSkeEvent{2005}{FungSR05}
    \newSkeEvent{2005}{ChavesVT05}
    \newSkeEvent{2005}{Torres2005}
    \newSkeEvent{2006}{EtchellsL06}
    \newSkeEvent{2006}{He2006}
    \newSkeEvent{2006}{huysmans2006iter}
    \newSkeEvent{2007}{BaderHM07}
    \newSkeEvent{2007}{SchetininFPCKEBH07}
    \newSkeEvent{2007}{ChenLW07}
    \newSkeEvent{2007}{BarakatB07}
    \newSkeEvent{2007}{SaadW07}
    \newSkeEvent{2007}{MartensBHVSB07}
    \newSkeEvent{2008}{NunezAC08}
    \newSkeEvent{2008}{SetionoBM08}
    \newSkeEvent{2008}{OdajimaHTS08}
    \newSkeEvent{2008}{grex-icdm2008}
    \newSkeEvent{2009}{Bader09}
    \newSkeEvent{2009}{MartensBG09}
    \newSkeEvent{2010}{LehmannBH10}
    \newSkeEvent{2012}{AugastaK12}
    \newSkeEvent{2012}{sethi2012kdruleex}
    \newSkeEvent{2016}{ZilkeMJ16}
    \newSkeEvent{2017}{ChanC17}
    \newSkeEvent{2018}{YedjourB18}
    \newSkeEvent{2020}{CHAN2020329}
    \newSkeEvent{2020}{WangWWYWJ20}
    \newSkeEvent{2021}{gridex-extraamas2021}
\end{chronology}
\end{landscape}

==> figures/tree-example.tex <==
% !TeX root = ../acmcs-skeskislr.tex

\begin{figure}
	\centering
	\begin{tikzpicture}%[grow=right,child anchor=west]
		\node[condition]{$\texttt{condition}_1$}
		child {
			node[decision]{$\texttt{output}_1$} edge from parent node[above left, pos = 0.7] {$True$}
		}
		child {
			node [condition]{$\texttt{condition}_2$} edge from parent {
				child {
					node[decision]{$\texttt{output}_2$} edge from parent node[above left, pos = 0.7] {$True$}
				}
				child {
					node[decision]{$\texttt{output}_3$} edge from parent node[above right, pos = 0.7] {$False$}
				}
				node[above right, pos = 0.7] {$False$}
			}
		};
	\end{tikzpicture}
	\caption{Example of output knowledge represented as a decision tree.}
	\label{fig:tree-example}
\end{figure}


==> figures/workflow.tex <==
% !TeX root = ../acmcs-skeskislr.tex

\begin{figure}
	\centering
	\begin{tikzpicture}%[grow=right,child anchor=west]
		\node[entity] (DS) at (0, 0) {Data set};
		\node[entity] (P) at (5, 0.8) {Predictor};
		\node[entity] (E) at (12, 2) {Extractor};
		\node[entity] (TR) at (8.5, 2) {Training\\set};
		\node[entity] (TE) at (3, -5) {Test set};
		
		\node[action] (FE) at (0, 2) {Feature\\engineering};
		\node[action] (SP) at (3, 2) {Train/test\\splitting};
		\node[action] (PT) at (5, -1) {Predictor\\training};		
		\node[action] (PP) at (8.5, -1) {Predictor\\pruning};
		\node[action] (KE) at (12, -1) {Knowledge\\extraction};
		\node[action] (KP) at (12, -5) {Knowledge\\pruning};		
		\node[action] (KF) at (8.5, -3) {Knowledge\\fixing};
		\node[action] (KI) at (5, -3) {Knowledge\\fixing};
		\node[action] (PA) at (8.5, -5) {Performance\\assessment};				
		
		\draw [->] (DS) -- (FE);
		\draw [->] (FE) -- (SP);
		\draw [->] (SP) -- (TR);
		\draw [->] (SP) -- (TE);
		\draw [->] (TR) -- (PT);
		\draw [->] (TE) -- (PA);
		\draw [->] (P) -- (PT);
		\draw [loop] (PT) -- (PP);
		\draw [loop] (PP) -- (KE);
		\draw [->] (E) -- (KE);
		\draw [->] (TR) -- (KE);
		\draw [loop] (KE) -- (KP);
		\draw [loop] (KP) -- (PA);
		\draw [loop] (PA) -- (KF);
		\draw [loop] (KF) -- (KI);
		\draw [loop] (KI) -- (PT);
	\end{tikzpicture}
	\caption{General structure of the train-extract-fix-inject loop.}
	\label{fig:ml-workflow-ske-ski}
\end{figure}


==> tables/fol-grammar.tex <==
% !TeX root = ../acmcs-skeskislr.tex

\begin{table}
    $$\begin{array}{rcl}
        \meta{Formula} & := & \meta{Clause} \mid \meta{Quantifier} \meta{Formula}
        \\
        \meta{Quantifier} & := & \terminal{\forall} \meta{Variable} \mid \terminal{\exists} \meta{Variable}
        \\
        \meta{Clause} & := & \meta{Literal} \mid \terminal{(} \meta{Formula} \meta{Connective} \meta{Formula} \terminal{)}
        \\
        \meta{Connective} & := & \terminal{\wedge} \mid \terminal{\vee} \mid \terminal{\rightarrow} \mid \terminal{\leftrightarrow} \mid \terminal{=}
        \\
        \meta{Literal}  & := & \meta{Predicate} \mid \terminal{\lnot} \meta{Predicate}
        \\
        \meta{Predicate} & := & \terminal{\top} \mid \terminal{\bot} \mid \meta{Predication} \mid \meta{Predication} \terminal{(} \meta{Arguments} \terminal{)}
        \\
        \meta{Predication} & := & p_1 \mid p_2 \mid p_3 \mid \ldots
        \\
        \meta{Arguments} & := & \meta{Term} \mid \meta{Term} \terminal{,} \meta{Arguments}
        \\
        \meta{Term} & := & \meta{Variable} \mid \meta{Structure} \mid \meta{Constant}
        \\
        \meta{Variable} & := & X_1 \mid X_2 \mid X_3 \mid \ldots
        \\
        \meta{Structure} & := & \meta{Functor} \terminal{(} \meta{Arguments} \terminal{)}
        \\
        \meta{Functor} & := & \functor{f}_1 \mid \functor{f}_2 \mid \functor{f}_3 \mid \ldots
        \\
        \meta{Constant} & := & \meta{Functor} \mid \meta{Number}\mid \meta{Boolean}
        \\
        \meta{Number} & := & \mathbb{R}
    \end{array}$$
    \caption[Context-free grammar for FOL]{Context-free grammar for FOL. Sans-serif words among angular brackets denote non-terminal symbols, whereas symbols among single apices denote terminal symbols.}
    \label{tab:fol-grammar}
\end{table}
